Linear stability analysis of detonations via numerical computation and dynamic mode decomposition

We introduce a new method to investigate linear stability of gaseous detonations that is based on an accurate shock-fitting numerical integration of the linearized reactive Euler equations with a subsequent analysis of the computed solution via the dynamic mode decomposition. The method is applied to the detonation models based on both the standard one-step Arrhenius kinetics and two-step exothermic-endothermic reaction kinetics. Stability spectra for all cases are computed and analyzed. The new approach is shown to be a viable alternative to the traditional normal-mode analysis used in detonation theory.

==> figures/verification.tex <==
\begin{tabular}{lcccccccc} \\
\toprule
$N_{1/2}$ & 20 & 40 & 80 & 160 & 320 & 640 & 1280 & 2560 \\
$E$ & {N/A}    & \num{   3e-02} & \num{   9e-04} & \num{   3e-05} & \num{   9e-07} & \num{   3e-08} & \num{   1e-09} & \num{   4e-11} \\
$r_{\text{acc}}$ & {N/A} & {N/A} & 5.07 & 4.96 & 5.00 & 5.00 & 4.81 & 4.57 \\
\bottomrule
\end{tabular}

